Instance-aware Exploration-Verification-Exploitation for Instance ImageGoal Navigation

As a new embodied vision task, Instance ImageGoal Navigation (IIN) aims to navigate to a specified object depicted by a goal image in an unexplored environment. The main challenge of this task lies in identifying the target object from different viewpoints while rejecting similar distractors. Existing ImageGoal Navigation methods usually adopt the simple Exploration-Exploitation framework and ignore the identification of specific instance during navigation. In this work, we propose to imitate the human behaviour of ``getting closer to confirm" when distinguishing objects from a distance. Specifically, we design a new modular navigation framework named Instance-aware Exploration-Verification-Exploitation (IEVE) for instance-level image goal navigation. Our method allows for active switching among the exploration, verification, and exploitation actions, thereby facilitating the agent in making reasonable decisions under different situations. On the challenging HabitatMatterport 3D semantic (HM3D-SEM) dataset, our method surpasses previous state-of-the-art work, with a classical segmentation model (0.684 vs. 0.561 success) or a robust model (0.702 vs. 0.561 success)

==> sections/results.tex <==
\section{Results}


\input{tables/dataset}

{\bf IEVE outperforms prior State-of-the-art.} The previous state-of-the-art work: \texttt{Mod-IIN} \cite{krantz2023navigating} achieved $0.561$ \textit{success} and $0.233$ \textit{SPL}, and we surpass their results in \textit{success} with a substantial margin of $0.105$ by attaining $0.666$ \textit{success} and a marginal improvement in \textit{SPL} with the help of a small visual backbone trained with Mask RCNN. Additionally, with the current state-of-the-art Semantic Segmentation model \texttt{InternImage}, our results are notably superior with an impressive score of $0.702$ \textit{success} and $0.252$ \textit{SPL}. This strongly demonstrates the pivotal role played by our Switch Policy in the success of navigation. However, we must acknowledge that our model fails to significantly enhance the agent's navigation efficiency, as evidenced by the relatively modest result in \textit{SPL}. We attribute this limitation to the Exploration Policy. In the ablation study, it is evident from \cref{tab:ablations} that the RL-trained policy does not perform superior to the random exploration policy. We contend that there exists a notable disparity between the current semantic map and the exploration goal map, as the agent requires additional information to comprehend the context of the construction of houses and enhance the efficiency of navigation. Instead of directly maximizing the coverage of the explored area, which is not distinct from the off-the-shelf frontier exploration policy.

{\bf Investigation into the impact of exploration policy.} From the tabular analysis presented in \cref{tab:ablations}, a comparison between the RL and random exploration policy provides us with valuable insights into the effectiveness and efficiency of RL in navigation. However, it is evident that RL policy yields marginal benefits in \textit{SPL} compared to frontier exploration policy. In particular, the margin of superiority for RL Policy over Frontier Exploration is significant at $0.053$ in \textit{SPL}. This disparity in performance is primarily due to the fact that exploring the entirety of a given environment can be time-consuming and unnecessary in most cases. Rather, the focus should be on gaining a comprehensive understanding of the most salient aspects of a small room, which can facilitate the identification of the target object. Furthermore, it is crucial for future research to leverage the concept of a knowledge graph, incorporating prior knowledge about the likely location of target objects, such as a refrigerator in the kitchen. By incorporating such information into the exploration process, we can further enhance the efficiency and efficacy of exploration.

{\bf Exploration-Verification-Exploitation benefits Navigation.} We conduct experiment about the impact of our Exploration-Verification-Exploitation (EVE) Policy on ultimate \textit{success} and \textit{SPL}. As depicted in the ablations table \cref{tab:ablations}, our EVE policy outperforms Exploration-Exploitation (EE) Policy by a substantial margin both in \textit{success} and \textit{SPL}. Specifically, \textit{success} from $0.590$ to $0.666$ and \textit{SPL} from $0.221$ to $0.235$. This suggests that the EVE policy provides the agent with greater opportunities to discern the current observation from the goal image, rather than arbitrarily assigning a false label to the current observed object in the EE policy.

{\bf Navigation benefits from instance segmentation.} From \cref{tab:ablations}, we can observe that state-of-the-art semantic segmentation model \texttt{InternImage} indeed benefits navigation, and also the ground truth segmented observation gives the upper bound of navigation. Specifically, more precisely segmented observation from \texttt{InternImage} gives higher metrics both in \textit{success} and \textit{SPL}. This is due to the more precise goal localization and less wrong segmentation results.


{\bf Euclidean distance from agent to the nearest goal point greatly influences instance re-identification.} From \cref{tab:reidentity}, it is evident that with a fixed threshold of $60$, the TP values for the difficulty level decrease significantly, from a high of $0.651$ in the easy level, to $0.569$ in the medium level, and eventually to $0.380$ in the hard level. It becomes more evident in the hard level with a threshold of $100$ that yields only $0.090$ of TP! This highlights the importance of careful examination and decision-making beyond the mere utilization of local feature algorithms to differentiate between similar objects. By meticulously examining the possible object instance, the agent is able to confidently arrive at a decision. We believe this explains why our model significantly surpasses previous state-of-the-art research in terms of \textit{Success} and achieves superior performance.

==> tables/ablation_exploration.tex <==
\setlength{\tabcolsep}{2.4pt}
\begin{table}[t]
    \centering
    {\small
\caption{\small Results}
\label{tab:1}
\vspace{-10pt}

\begin{tabular}{lcccccccccccccc}
\toprule
 & & \multicolumn{2}{c}{Dataset params} & & \multicolumn{2}{c}{Discriminator params} & & \multicolumn{6}{c}{Predictions}   \\ 
 Methods & & Min\_dis & Max\_dis & & MatchedPoints & CheckDistance & & TP & TN & MP & MN & FP & FN  \\ \midrule
 FeaturMatching & & 0 &  2 & & 30 & - & & 5554(0.819) & 1366(0.327) & - & - & 1226(0.181) & 2816(0.673) \\
 FeaturMatching & & 0 &  2 & & 20 & - & & 6140(0.906) & 2573(0.615) & - & - & 640(0.094) & 1609(0.385) \\
 FeaturMatching & & 0 &  2 & & 15 & - & & 6347(0.936) & 3206(0.767) & - & - & 433(0.064) & 976(0.233) \\
 FeaturMatching & & 0 &  2 & & 25 & - & & 6362(0.938) & 3206(0.767) & - & - & 418(0.062) & 976(0.233) \\
 FeaturMatching & & 2 &  4 & & 25 & - & & 4360(0.822) & 1829(0.464) & - & - & 941(0.178) & 2110(0.536) \\
 FeaturMatching & & 4 &  6 & & 25 & - & & 557(0.722) & 244(0.444) & - & - & 215(0.278) & 305(0.556) \\
 FeaturMatching & & 0 &  4 & & 40 & - & & 8558(0.708) & 1298(0.139) & - & - & 3529(0.292) & 8056(0.861) \\
 FeaturMatching & & 0 &  2 & & 60 & - & & 7329(0.606) & 329(0.035) & - & - & 4758(0.394) & 9025(0.965) \\
 HeuristicMatching & & 2 &  4 & & 25 & 3 & & 3947(0.796) & 753(0.207) & 345 & 302 & 1009(0.204) & 2884(0.793) \\
 HeuristicMatching & & 4 &  6 & & 25 & 3 & & 4269(0.790) & 828(0.198) & 681 & 337 & 1133(0.210) & 3360(0.802) \\ \bottomrule

\end{tabular}    }
\end{table}

==> tables/dataset.tex <==
% \begin{table*}
%   \centering
%   \begin{tabular}{@{}ccccccccccccc@{}}
%     \toprule
%     & \multicolumn{4}{c}{\textbf{Easy}} & \multicolumn{4}{c}{\textbf{Medium}} & \multicolumn{4}{c}{\textbf{Hard}} \\
%     \cmidrule(2-11)
%     Thresh & TP(easy) & TN(easy) & FP(easy) & FN(easy) & TP(medium) & TN(medium) & FP(medium) & FN(medium) & TP(hard) & TN(hard) & FP(hard) & FN(hard) \\
%     \midrule
%     40 & 0.741 & 0.853 & 0.259 & 0.147 & 0.569 & 0.965 & 0.431 & 0.035 & 0.526 & 0.835 & 0.474 & 0.165 \\
%     60 & 0.651 & 0.963 & 0.349 & 0.037 & 0.569 & 0.964 & 0.431 & 0.036 & 0.380 & 0.961 & 0.620 & 0.039 \\
%     80 & 0.610 & 0.977 & 0.390 & 0.023 & 0.500 & 0.982 & 0.500 & 0.018 & 0.314 & 0.974 & 0.686 & 0.026 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Euclidean distance and matched points' influence on decision-making. We utilize our Instance Re-Identification dataset to illustrate euclidean distance and matched keypoints' impact on re-identifying a particular object on the goal image.}
%   \label{tab:reidentity}
% \end{table*}

\begin{table*}
  \centering
  \begin{tabular}{@{}ccccccccccccc@{}}
    \toprule
    & \multicolumn{4}{c}{\textbf{Easy}} & \multicolumn{4}{c}{\textbf{Medium}} & \multicolumn{4}{c}{\textbf{Hard}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    Thresh & TP & TN & FN & FP & TP & TN & FN & FP & TP & TN & FN & FP \\
    \midrule
    % \midrule
    40 & 0.741 & 0.853 & 0.259 & 0.147 & 0.569 & 0.848 & 0.431 & 0.152 & 0.526 & 0.835 & 0.474 & 0.165 \\
    60 & 0.651 & 0.963 & 0.349 & 0.037 & 0.569 & 0.964 & 0.431 & 0.036 & 0.380 & 0.961 & 0.620 & 0.039 \\
    80 & 0.610 & 0.977 & 0.390 & 0.023 & 0.500 & 0.982 & 0.500 & 0.018 & 0.314 & 0.974 & 0.686 & 0.026 \\
    100 & 0.582 & 0.981 & 0.418 & 0.019 & 0.451 & 0.986 & 0.549 & 0.014 & 0.090 & 0.992 & 0.910 & 0.008 \\
    \bottomrule
  \end{tabular}
  \caption{The probabilities of TP, TN, FP, and FN under various difficulty levels (according to the Euclidean distance between the agent and potential target) and selected thresholds (the number of matched keypoints).}
  \label{tab:reidentity}
  \vspace{-10pt}
\end{table*}

==> tables/instance_classify.tex <==

\setlength{\tabcolsep}{.3em}
\begin{table}[t]
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \renewcommand{\arraystretch}{1.15}
    \begin{center}
	\resizebox{1.00\columnwidth}{!}{
		\begin{tabular}{cll ccsc}
			\toprule
            & \multicolumn{2}{c}{\scriptsize\textbf{Model Variation}}
			& \multicolumn{4}{c}{\scriptsize\textbf{Validation}}
            \\
			\cmidrule{4-7}
			\scriptsize \shortstack{\#} &
			Instance Re-ID
                & Goal Localization
			& \scriptsize\textbf{\texttt{NE}}~$\downarrow$
			& \scriptsize\textbf{\texttt{Max-ST}}~$\downarrow$
			& \scriptsize\textbf{\texttt{SR}}~$\uparrow$
			& \scriptsize\textbf{\texttt{SPL}}~$\uparrow$
			\\
			\midrule
			\scriptsize \texttt{1}
                    & Keypoint-Conf
                    & Detic-Projected
                    &  \textbf{3.096}  & \textbf{0.310} & \textbf{0.561}  &  \textbf{0.233}
                    \\
			\scriptsize \texttt{2}
                    & Keypoint-Match
                    & Detic-Projected
                    &  3.261  & 0.339 & 0.539  &  0.221
                    \\
			\scriptsize \texttt{3}
                    & Keypoint-Conf
                    & Crop-Projected
                    &  3.128  & 0.301 & 0.523  &  0.224
                    \\
			\scriptsize \texttt{4}
                    & Keypoint-Conf
                    & Detic-ObjectNav
                    &  3.235  & 0.327 & 0.488  &  0.205
                    \\
			\scriptsize \texttt{5}
                    & ResNet
                    & Detic-ObjectNav
                    &  6.264  & 0.857 & 0.138  &  0.044
                    \\
			\scriptsize \texttt{6}
                    & CLIP
                    & Detic-ObjectNav
                    &  6.570  & 0.917 & 0.097  &  0.029
                    \\
			\midrule
			\scriptsize \texttt{7}
                    & Oracle
                    & Oracle
                    &  1.300  & 0.089 & 0.845  &  0.453
                    \\
			\scriptsize \texttt{8}
                    & Oracle
                    & Detic-Projected
                    &  2.551  & 0.116 & 0.498  &  0.250
                    \\
			\scriptsize \texttt{9}
                    & Keypoint-Conf
                    & Oracle
                    &  2.914  & 0.348 & 0.647  &  0.266
                    \\
			\bottomrule
		\end{tabular}}
	\end{center}
	\caption{Our Modular InstanceImageNav method (\texttt{Mod-IIN}: row 1) with variations to instance re-identification and goal localization. }
	\label{tab:ablations}
\end{table}


==> tables/reb_1.tex <==
\begin{table}[t]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{cccccc}
    \toprule
    \multicolumn{4}{c}{\textbf{Model Variation}} & \multicolumn{2}{c}{\textbf{Validation}} \\
    \cmidrule{5-6}
    % \rowcolor{lightgray}
    Classification & Perception & Switch & Exploration & \textit{Success}~$\uparrow$ & \textit{SPL}~$\uparrow$ \\
    \midrule
    % \midrule
    Mask RCNN & Mask RCNN & EVE & RL & 0.666 & 0.235  \\
    % \rowcolor{lightgray!50}
    Mask RCNN & Mask RCNN & EVE & Frontier & 0.676 & 0.182 \\
    Mask RCNN & Mask RCNN & EVE & Random & 0.654 & 0.233 \\
    % \rowcolor{lightgray!50}
    Mask RCNN & Mask RCNN & EE & RL & 0.590 & 0.221 \\
    InternImage & InternImage & EVE & RL & \textbf{0.702} & \textbf{0.252} \\
    \midrule
    SwinTrans & Mask RCNN & EVE & RL & \textbf{0.684} & \textbf{0.241}  \\
    % \rowcolor{lightgray!50}
    SwinTrans & Mask RCNN & EVE & Frontier & 0.628 & 0.180 \\
    SwinTrans & Mask RCNN & EVE & Random & 0.636 & 0.236 \\
    % \rowcolor{lightgray!50}
    SwinTrans & Mask RCNN & EE & RL & 0.620 & 0.216 \\
    SwinTrans & InternImage & EVE & RL & 0.676 & 0.238 \\
    \midrule
    % \rowcolor{lightgray!50}
    GroundTruth & Mask RCNN & EVE & RL & 0.682 & 0.238 \\
    GroundTruth & Oracle & - & RL & 0.850 & 0.399 \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-6pt}
  \caption{Hyperparameters' impact of GMS on the success and SPL of navigation}
  \vspace{-10pt}
  \label{tab:reb_1}

\end{table}

==> tables/total.tex <==
\begin{table}
  \centering
  \begin{subtable}[t]{0.4\linewidth}
  \begin{tabular}{@{}ccc@{}}
    \toprule
    & \multicolumn{2}{c}{\textbf{Validation}} \\
    \cmidrule{2-3}
    Model & \texttt{Success}~$\uparrow$ & \texttt{SPL}~$\uparrow$ \\
    \midrule
    \texttt{RL Baseline} & 0.083 & 0.035  \\
    \texttt{OVRL-v2 ImageNav} & 0.006 & 0.002 \\
    \texttt{OVRL-v2 InstanceImageNav} & 0.248 & 0.118 \\
    \texttt{Mod-IIN} & 0.561 & 0.233 \\
    \texttt{IEVE (Mask RCNN)} & 0.666 & 0.235 \\
    \texttt{IEVE (InternImage)} & \textbf{0.702} & \textbf{0.252} \\
    \bottomrule
  \end{tabular}
  \caption{We compare our Instance-oriented Exploration-Verification-Exploitation \texttt{IEVE} against prior methods on Instance ImageGoal Navigation. \texttt{IEVE} outperforms the baseline model (row 1) with up to $8.75$x increase in \texttt{Success} and outperforms a state-of-the-art model \cite{krantz2023navigating} (\texttt{Mod-IIN}, row 4) from $0.561$ to $0.666$ with a lightweight segmentation model (Mask RCNN) on \texttt{Success}, and higher \texttt{Success} of $0.702$ with a strong backbone (InternImage \cite{wang2023internimage}).}
  \label{tab:main}
  \end{subtable}
\end{table}
